Leveraging Software Architectures to Guide and Verify the Development of Sense/Compute/Control Applications

A software architecture describes the structure of a computing system by specifying software components and their interactions. Mapping a software architecture to an implementation is a well known challenge. A key element of this mapping is the architecture's description of the data and control-flow interactions between components. The characterization of these interactions can be rather abstract or very concrete, providing more or less implementation guidance, programming support, and static verification. In this paper, we explore one point in the design space between abstract and concrete component interaction specifications. We introduce a notion of behavioral contract that expresses the set of allowed interactions between components, describing both data and control-flow constraints. This declaration is part of the architecture description, allows generation of extensive programming support, and enables various verifications. We instantiate our approach in an architecture description language for the domain of Sense/Compute/Control applications, and describe associated compilation and verification strategies.

==> code/LighttpdAccessLogParser.tex <==
% Remember to use the lgrind style

\Head{}
\File{LighttpdAccessLogParser.java}{2011}{2}{11}{12:13}{528}
\L{\LB{\K{public}_\K{class}_\V{LighttpdAccessLogParser}}}
\L{\LB{}\Tab{19}{\K{extends}_\V{AbstractAccessLogParser}_\{}}
\L{\LB{}\Tab{4}{@\V{Override}}}
\index{onNewLine}\Proc{onNewLine}\L{\LB{}\Tab{4}{\K{public}_\V{Access}_\V{onNewLine}(\V{String}_\V{newLine})_\{}}
\L{\LB{}\Tab{8}{\V{Access}_\V{access}_=_\K{new}_\V{Access}();}}
\L{\LB{}\Tab{8}{\V{access}.\V{setLine}(\V{newLine});}}
\L{\LB{}\Tab{8}{\V{access}.\V{setHost\_ip}(\V{parseRemoteHostIP}(\V{newLine}));}}
\L{\LB{}\Tab{8}{.\,.\,._\C{}//_parsing_of_the_other_fields\CE{}}}
\L{\LB{}\Tab{8}{\K{return}_\V{access};}}
\L{\LB{}\Tab{4}{\}}}
\L{\LB{}}
\index{parseRemoteHostIP}\Proc{parseRemoteHostIP}\L{\LB{}\Tab{4}{\K{private}_\V{IPAddress}_\V{parseRemoteHostIP}(\V{String}_\V{newLine})_\{}}
\L{\LB{}\Tab{8}{\V{Pattern}_\V{pattern}_=_\V{Pattern}.\V{compile}(\S{}\3\5([\5_]+)_\3\SE{});}}
\L{\LB{}\Tab{8}{\V{Matcher}_\V{m}_=_\V{pattern}.\V{matcher}(\V{newLine});}}
\L{\LB{}\Tab{8}{\V{m}.\V{find}();}}
\L{\LB{}\Tab{8}{\K{return}_\K{new}_\V{IPAddress}(\V{m}.\V{group}(\N{1}));}}
\L{\LB{}\Tab{4}{\}}}
\L{\LB{\}}}


==> code/accessprofile.tex <==
% Remember to use the lgrind style

\Head{}
\File{accessprofile.java}{2010}{5}{27}{11:43}{333}
\L{\LB{\K{public}_\K{class}_\V{AccessingProfile}_\K{extends}_\V{AbstractAccessingProfile}_\{}}
\L{\LB{}}
\L{\LB{}\Tab{2}{@\V{Override}}}
\L{\LB{}\Tab{2}{\K{protected}_\V{IdentifiedAccess}}}
\index{onNewAccessLogParser}\Proc{onNewAccessLogParser}\L{\LB{}\Tab{2}{\V{onNewAccessLogParser}(\V{Access}_\V{newAccess},}}
\L{\LB{}\Tab{23}{\V{PullFromIP2ProfileCallback}_\V{ip2Profile})_\{}}
\L{\LB{}\Tab{4}{\V{Profile}_\V{profile}_=_\V{ip2Profile}.\V{get}(\V{newAccess}.\V{getHost\_ip}());}}
\L{\LB{}\Tab{4}{\K{return}_\K{new}_\V{IdentifiedAccess}(\V{newAccess},_\V{profile});}}
\L{\LB{}\Tab{2}{\}}}
\L{\LB{\}}}


==> code/dynguard.tex <==
% Remember to use the lgrind style

\Head{}
\File{dynguard.java}{2010}{5}{26}{19:52}{1112}
\L{\LB{\K{public}_\K{abstract}_\K{class}_\V{AbstractAccessingProfile}_\{}}
\L{\LB{}\Tab{2}{\C{}//_the_callback{'}s_internal_class\CE{}}}
\L{\LB{}\Tab{2}{\K{protected}_\K{class}_\V{PullFromIP2ProfileCallback}_\{}}
\L{\LB{}\Tab{4}{\K{private}_\K{boolean}_\V{isActive}_=_\K{false};_\C{}//_the_dynamic_guard\CE{}}}
\L{\LB{}\Tab{4}{\C{}//_the_callback_method\CE{}}}
\index{get}\Proc{get}\L{\LB{}\Tab{4}{\K{public}_\V{Profile}_\V{get}(\V{IPAddress}_\V{ipAddress})_\{}}
\L{\LB{}\Tab{6}{\K{if}_(!\V{isActive})}}
\L{\LB{}\Tab{8}{\K{throw}_\K{new}_\V{IllegalAccessError}(\S{}\3Illegal_call\3\SE{});}}
\L{\LB{}\Tab{6}{\C{}//_pull_the_value_from_the_instance_of_IP2Profile\CE{}}}
\L{\LB{}\Tab{6}{\C{}//_through_a_call_to_the_underlying_middleware\CE{}}}
\L{\LB{}\Tab{6}{\K{return}_.\,.\,.;}}
\L{\LB{}\Tab{4}{\}}}
\L{\LB{}\Tab{2}{\}}}
\L{\LB{}}
\L{\LB{}\Tab{2}{\C{}//_the_calling_method\CE{}}}
\index{callOnNewAccessLogParser}\Proc{callOnNewAccessLogParser}\L{\LB{}\Tab{2}{\K{private}_\K{void}_\V{callOnNewAccessLogParser}(\V{Access}_\V{value})_\{}}
\L{\LB{}\Tab{4}{\V{PullFromIP2ProfileCallback}_\V{c}_=_\K{new}_\V{PullFromIP2ProfileCallback}();}}
\L{\LB{}\Tab{4}{\V{c}.\V{isActive}_=_\K{true};_\C{}//_dynamic_guard_deactivation\CE{}}}
\L{\LB{}}
\L{\LB{}\Tab{4}{\V{IdentifiedAccess}_\V{newValue};}}
\L{\LB{}\Tab{4}{\K{try}_\{}}
\L{\LB{}\Tab{6}{\C{}//_calls_the_developer{'}s_method\CE{}}}
\L{\LB{}\Tab{6}{\V{newValue}_=_\V{onNewAccessLogParser}(\V{value},_\V{c});}}
\L{\LB{}\Tab{4}{\}_\K{finally}_\{}}
\L{\LB{}\Tab{6}{\V{c}.\V{isActive}_=_\K{false};_\C{}//_dynamic_guard_activation\CE{}}}
\L{\LB{}\Tab{4}{\}}}
\L{\LB{}\Tab{4}{\C{}//_publish_newValue_by_using_the_underlying_middleware\CE{}}}
\L{\LB{}\Tab{4}{.\,.\,.}}
\L{\LB{}\Tab{2}{\}}}
\L{\LB{}}
\index{onNewAccessLogParser}\Proc{onNewAccessLogParser}\L{\LB{}\Tab{2}{\K{protected}_\K{abstract}_\V{IdentifiedAccess}_\V{onNewAccessLogParser}(}}
\L{\LB{}\Tab{11}{\V{Access}_\V{newAccessLogParser},}}
\L{\LB{}\Tab{11}{\V{PullFromIP2ProfileCallback}_\V{ip2Profile});}}
\L{\LB{}\Tab{2}{.\,.\,.}}
\L{\LB{\}}}

